Control of Discrete-Time LTI Systems using Stochastic Ensemble Systems

In this paper, we study the control properties of a new class of stochastic ensemble systems that consists of families of random variables. These random variables provide an increasingly good approximation of an unknown discrete, linear-time invariant (DLTI) system, and can be obtained by a standard, data-driven procedure. Our first result relates the reachability properties of the stochastic ensemble system with that of the limiting DLTI system. We then provide a method to combine the control inputs obtained from the stochastic ensemble systems to compute a control input for the DLTI system. Later, we deal with a particular kind of stochastic ensemble system generated from realizing Bernoulli random variables. For this, we characterize the variance of the computed state and control. We also do the same for a situation where the data is updated sequentially in a streaming fashion. We illustrate the results numerically in various simulation examples.

==> macros-abbrev.tex <==
%% Macros for Coordination book
\newcommand{\ds}{\displaystyle}

%%%% enumerate environment containing text and with un-interrupted numbering
\newcounter{saveenum}
%% \setcounter{saveenum}{\value{enumi}}
%% \setcounter{enumi}{\value{saveenum}}

% abbreviations
\newcommand\ie{\mbox{i.e.,\xspace}}
\newcommand\eg{\mbox{e.g.,\xspace}}
\newcommand\etal{\mbox{et~al.,\xspace}}
\newcommand\etc{\mbox{etc.\@\xspace}}
\newcommand\cf{\mbox{cf.\@\xspace}}
\newcommand\resp{\mbox{resp.\@\xspace}}

\newcommand{\e}{\operatorname{e}}

%% Set definitions
\renewcommand{\natural}{{\mathbb{N}}}
\newcommand{\integer}{\ensuremath{\mathbb{Z}}}
\newcommand{\integernonnegative}{\ensuremath{\mathbb{Z}}_{\ge 0}}
\newcommand{\naturalzero}{\integernonnegative} % redundant, to remove
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\realpositive}{\ensuremath{\mathbb{R}}_{>0}}
\newcommand{\realnonnegative}{\ensuremath{\mathbb{R}}_{\ge 0}}
\newcommand{\complex}{\ensuremath{\mathbb{C}}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\SO}[1]{\mathrm{SO}(#1)}
\newcommand{\SE}[1]{\mathrm{SE}(#1)}
%% Set operations
\newcommand{\union}{\operatorname{\cup}}
\newcommand{\intersection}{\ensuremath{\operatorname{\cap}}}
\newcommand{\intersect}{\ensuremath{\operatorname{\cap}}}
\newcommand{\bigintersect}{\bigcap}

%% mathematical constructs: \setdef, \until, etc
\newcommand{\until}[1]{\{1,\dots, #1\}}
\newcommand{\subscr}[2]{#1_{\textup{#2}}}
\newcommand{\supscr}[2]{#1^{\textup{#2}}}
\newcommand{\setdef}[2]{\{#1 \; | \; #2\}}
\newcommand{\bigsetdef}[2]{\big\{#1 \; | \; #2\big\}}
\newcommand{\Bigsetdef}[2]{\Big\{#1 \; \big| \; #2\Big\}}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\setmap}[3]{#1: #2 \rightrightarrows #3}
\newcommand{\id}{\operatorname{id}}
\newcommand{\diag}[1]{\operatorname{diag}(#1)}
\newcommand{\setofsetvalued}[2]{\mathcal{SC}(#1,#2)}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\image}{\operatorname{image}}

%% mathematical functions
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\radius}{\operatorname{radius}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\wdist}{\operatorname{wdist}}
\newcommand{\interior}[1]{\operatorname{int}(#1)}
\newcommand{\oball}[2]{B(#1,#2)}
\newcommand{\bigoball}[2]{B\big(#1,#2\big)}
\newcommand{\Bigoball}[2]{B\Big(#1,#2\Big)}
\newcommand{\cball}[2]{\overline{B}(#1,#2)}
\newcommand{\bigcball}[2]{\overline{B}\big(#1,#2\big)}
\newcommand{\Bigcball}[2]{\overline{B}\Big(#1,#2\Big)}
\newcommand{\der}[2]{\frac{d #1}{d #2}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}

%% Symbols from Chp 2 Curves
\newcommand{\signedcurvature}{ \subscr{\kappa}{signed} }
\newcommand{\abscurvature}{ \subscr{\kappa}{abs} }
\newcommand{\radiuscurvature}{\rho}
\newcommand{\normalvector}{\operatorname{n}}
\newcommand{\innormalvector}{\operatorname{n}_{\textup{in}}}
\newcommand{\outnormalvector}{\operatorname{n}_{\textup{out}}}

%% Symbols from Chp 2 Matrix
\newcommand{\identitymatrix}[1]{I_{#1}}
\newcommand{\spectrum}{\operatorname{spec}}
\newcommand{\spectralradius}{\rho}
\newcommand{\essspectralradius}{\subscr{\rho}{ess}}

%% Symbols from Chp 2 Distributed Algorithms
\newcommand{\parts}[1]{\mathbb{P}(#1)}
\newcommand{\finite}[1]{\mathbb{F}(#1)} 
%%% make sure there are no 2^X in the final document
\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\vectorones}[1][]{\vect{1}_{#1}}
\newcommand{\vectorzeros}[1][]{\vect{0}_{#1}}
\newcommand{\kernel}{\operatorname{kernel}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\proj}{\operatorname{proj}}

%% graph
\newcommand{\graph}{G}
\newcommand{\vertices}{V}
\newcommand{\edges}{E}
\newcommand{\adjmat}{A}
\newcommand{\neighbors}{\mathcal{N}}
\newcommand{\neighborsin}{\mathcal{N}^{\textup{in}}}
\newcommand{\neighborsout}{\mathcal{N}^{\textup{out}}}
\newcommand{\length}{\operatorname{length}}
\newcommand{\weight}{\operatorname{weight}}
\newcommand{\reverse}{\operatorname{rev}}
\newcommand{\TBFS}{\ensuremath{\subscr{T}{BFS}}\xspace}
\newcommand{\TDFS}{\ensuremath{\subscr{T}{DFS}}\xspace}
\newcommand{\Tshpt}{\ensuremath{\subscr{T}{shortest-paths}}\xspace}
%% \newcommand{\TMST}{\ensuremath{\subscr{T}{MST}}\xspace}
%% \newcommand{\TSP}{\ensuremath{\subscr{T}{TSP}}\xspace}
\newcommand{\algofont}[1]{\textsc{#1}}
\newcommand{\algostep}[1]{{\small\texttt{#1:}}\xspace}

%% Chp2: state machines and dynamical systems
\newcommand{\equilibria}[1]{\operatorname{Equil}(#1)}
\newcommand{\lieder}[2]{\mathcal{L}_{#1}#2}

%% Chp2: synchronous network
\newcommand{\network}[1][]{\mathcal{S}_{\textup{#1}}}
\newcommand{\Ecmm}{\subscr{E}{cmm}}

\newcommand{\alphabet}{\mathbb{A}}

%% robot and environment sensing: function, alphabet, symbol
\newcommand{\rbtsns}{\textup{rbt-sns}\xspace}
\newcommand{\rbtalphabet}{\subscr{\mathbb{A}}{rbt}}
\newcommand{\rbts}{y}

\newcommand{\envsns}{\textup{env-sns}\xspace}
\newcommand{\envalphabet}{\subscr{\mathbb{A}}{env}}
\newcommand{\envs}{\subscr{y}{env}}


\newcommand{\supind}[2]{{#1}^{[#2]}}
\newcommand{\superscr}[2]{{#1}^{\operatorname{#2}}}
\newcommand{\subind}[2]{{#1}_{[#2]}}
\newcommand{\DA}[1][]{\mathcal{D\!A}_{\textup{#1}}}
\newcommand{\timeschedule}{\integernonnegative}
\newcommand{\edtimeschedule}{\Sigma}
\newcommand{\nll}{\mytt{null}}
\newcommand{\msg}{\textup{msg}\xspace}
\newcommand{\stf}{\textup{stf}\xspace}
\newcommand{\msgtrig}{\textup{msg-trig}\xspace}
\newcommand{\stftrig}{\textup{stf-trig}\xspace}
\newcommand{\msggen}{\textup{msg-gen}\xspace}
\newcommand{\msgrec}{\textup{msg-rec}\xspace}
\newcommand{\msgstandard}{\textup{msg}_{\textup{std}}}
\newcommand{\TC}{\operatorname{TC}}
\newcommand{\SC}{\operatorname{SC}}
\newcommand{\CC}{\operatorname{CC}}

%% algorithmic enviroment fixes
\newcommand{\AND}{AND\xspace}
\newcommand{\OR}{OR\xspace}
\newcommand{\return}{\textbf{return}\xspace}
\newcommand{\mycase}{\textbf{case}\xspace}
\newcommand{\mytt}[1]{\textup{\texttt{#1}}\xspace} %% mytt = my typefont text
\newcommand{\true}{\mytt{true}}
\newcommand{\false}{\mytt{false}}
\newcommand{\data}{\mytt{data}}
\newcommand{\newdata}{\mytt{new-data}}
\newcommand{\leader}{\mytt{leader}}
\newcommand{\newleader}{\mytt{new-lead}}
\newcommand{\transmit}{\mytt{transmit}}
\newcommand{\newtransmit}{\mytt{new-transmit}}
\renewcommand{\transmit}{\mytt{snd-flag}}
\renewcommand{\newtransmit}{\mytt{new-snd-flag}}
\newcommand{\search}{\mytt{search}}
\newcommand{\newsearch}{\mytt{new-search}}
\newcommand{\round}{\mytt{round}}
\newcommand{\unknown}{\mytt{unknwn}}
\newcommand{\maxuid}{\mytt{max-id}}
\newcommand{\newuid}{\mytt{new-id}} 
\newcommand{\uid}{\mytt{uid}}
\newcommand{\uuu}{\mytt{my-id}}
\newcommand{\parent}{\mytt{parent}}
\newcommand{\newparent}{\mytt{new-parent}}
\newcommand{\mydist}{\mytt{dist}}
\newcommand{\newdist}{\mytt{new-dist}}
\newcommand{\mypar}{\mytt{parent}}

%% Chp2: linear iterations
\newcommand{\TwoNorm}[1]{\|#1\|_2}
\newcommand{\bigTwoNorm}[1]{\big \|#1 \big \|_2}
\newcommand{\BigTwoNorm}[1]{\Big \|#1 \Big \|_2}
\newcommand{\PNorm}[1]{\|#1\|_p}
\newcommand{\InftyNorm}[1]{\|#1\|_{\infty}}
\newcommand{\ymaxmin}{\subscr{y}{max-min}}
\newcommand{\yerr}{\subscr{y}{err}}
\newcommand{\expfac}{\subscr{r}{exp}}

\newcommand{\tridmat}{\operatorname{Trid}}
\newcommand{\atridmat}{\operatorname{ATrid}}
\newcommand{\circmat}{\operatorname{Circ}}
\newcommand{\yave}{\subscr{y}{ave}}
\newcommand{\xave}{\subscr{x}{ave}}
\newcommand{\zave}{\subscr{z}{ave}}

\newcommand{\complexnorm}[1]{\|#1\|_\complex}
\newcommand{\Bigcomplexnorm}[1]{\Big\|#1\Big\|_\complex}
\newcommand{\norm}[2]{\|#1\|_{#2}}
\newcommand{\bignorm}[2]{\big\|#1\big\|_{#2}}
\newcommand{\Bignorm}[2]{\Big\|#1\Big\|_{#2}}
\newcommand{\Biggnorm}[2]{\Bigg\|#1\Bigg\|_{#2}}
\newcommand{\Enorm}[1]{\|#1\|_{2}}

\newcommand{\ii}{i_{\mathbb{F}}}

%% proof of number theory result
\newcommand{\mquot}{\subscr{m}{qtnt}}
\newcommand{\mremain}{\subscr{m}{rmndr}}



%% Set of matrices
\newcommand{\stoch}[1]{{\cal F}(#1)}
\newcommand{\substoch}[2]{{\cal F}_{#2}(#1)}

%% Symbols from Chp 3 Geometry
\newcommand{\PP}{\mathcal{P}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\ov}{\overline}
\newcommand{\fti}{\operatorname{fti}}
\newcommand{\visibilityset}[2]{\operatorname{Vi}(#1;#2)}
%% \newcommand{\robustvisibilityset}[3]{\operatorname{Vi}_{#3}(#1;#2)}

%% range-limited visibility set; defined chapter 4 or 5
\newcommand{\rlvs}[2]{\subscr{\operatorname{Vi}}{disk}(#1;#2)}


%% distances
\newcommand{\distC}{\operatorname{\subscr{dist}{\texttt{c}}}}
\newcommand{\distCC}{\operatorname{\subscr{dist}{\texttt{cc}}}}

%% polytopes
\newcommand{\chull}[1]{\operatorname{co}(#1)}
\newcommand{\rchull}[2]{\operatorname{rco}_{#2}(#1)}
\renewcommand{\rchull}[2]{\operatorname{rco}(#1;#2)}
\newcommand{\co}{\operatorname{co}}

%% geometric centers
\newcommand{\ccenter}[1]{\operatorname{CC}(#1)}
\newcommand{\ccenterBig}[1]{\operatorname{CC}\!\big(#1\big)}
\newcommand{\icenter}[1]{\operatorname{IC}(#1)}
\newcommand{\cradius}[1]{\operatorname{CR}(#1)}
\newcommand{\iradius}[1]{\operatorname{IR}(#1)}
\newcommand{\area}[2]{\operatorname{A}_{#2}(#1)}
\newcommand{\centroid}[2]{\operatorname{CM}_{#2}(#1)}
\newcommand{\momentofinertia}[3]{\operatorname{J}_{#2}(#1,#3)}
\newcommand{\verticespolytope}[1]{\operatorname{Ve}(#1)}
\newcommand{\facetspolytope}[1]{\operatorname{Fa}(#1)}
\newcommand{\edgespolytope}[1]{\operatorname{Ed}(#1)}
\newcommand{\density}{\phi}
\newcommand{\Voronoi}[1]{\mathcal{V}(#1)}
\newcommand{\limVoronoi}[1]{\mathcal{V}_r(#1)}

%% proximity graphs
\newcommand{\proximitygraph}{\mathcal{G}} 
\newcommand{\edgesproximitygraph}[1]{\mathcal{E}_{#1}} 
\newcommand{\neighborsproximitygraph}{\mathcal{N}}
\newcommand{\completegraph}{\subscr{\proximitygraph}{cmplt}}
\newcommand{\rdiskgraph}{\subscr{\proximitygraph}{disk}(r)}
\newcommand{\ridiskgraph}{\subscr{\proximitygraph}{$\infty$-disk}(r)}
\newcommand{\Dgraph}{\subscr{\proximitygraph}{D}}
\newcommand{\rDgraph}[1]{\subscr{\proximitygraph}{LD}(#1)}
\newcommand{\aDgraph}{\subscr{\proximitygraph}{LD}(a)}
\newcommand{\RNgraph}{\subscr{\proximitygraph}{RN}}
\newcommand{\Ggraph}{\subscr{\proximitygraph}{G}}
\newcommand{\EMSTgraph}{\subscr{\proximitygraph}{EMST}}
\newcommand{\EMSTGgraph}[1]{\subscr{\proximitygraph}{EMST,$#1$}}
\newcommand{\Vgraph}[1]{\subscr{\proximitygraph}{vis,$#1$}}
\newcommand{\Vdiskgraph}[1]{\subscr{\proximitygraph}{vis-disk,$#1$}}
\newcommand{\ClessVdiskgraph}[1]{\subscr{\proximitygraph}{lc-vis-disk,$#1$}}
%% \newcommand{\RVgraph}{\subscr{\proximitygraph}{$\eps$-vis,Q}}
\newcommand{\LCgraph}[1]{\subscr{\proximitygraph}{lc,$#1$}}

\newcommand{\osegment}[2]{]#1,#2[}
\newcommand{\csegment}[2]{[#1,#2]}
\newcommand{\ocsegment}[2]{]#1,#2]}

%% geometric optimization
\newcommand{\HH}{\mathcal{H}}
\newcommand{\HHexp}{\mathcal{H}_{\textup{exp}}}
\newcommand{\HHdistor}{\mathcal{H}_{\textup{dist}}}
\newcommand{\HHarea}[1]{\mathcal{H}_{\textup{area},#1}}
\newcommand{\HHmixed}[1]{\mathcal{H}_{\textup{dist-area},#1}}
\newcommand{\HHworst}{\mathcal{H}_{\textup{worst}}}
\newcommand{\HHdc}{\mathcal{H}_{\textup{dc}}}
\newcommand{\HHsp}{\mathcal{H}_{\textup{sp}}}
\newcommand{\HHsum}{\mathcal{H}_\Sigma}
\newcommand{\HHmax}{\mathcal{H}_{\max}}
\newcommand{\performance}{f}
\newcommand{\coincident}{\mathcal{S}_{\textup{coinc}}}
\newcommand{\indicator}[1]{\operatorname{1}_{#1}}
\newcommand{\arc}{\operatorname{arc}}
\newcommand{\discont}[1]{\operatorname{Dscn}(#1)}

%% maybe to move into Chap 2
\newcommand{\scalarproduct}[2]{#1 \cdot #2}

%% Symbols from Chp 4 Model
\newcommand{\groupop}{\star}
\newcommand{\groupidentity}{e}
\newcommand{\so}{\mathfrak{so}}

%% Feedback communication and control + Tasks
\newcommand{\setofrobots}{\mathcal{R}}
\newcommand{\robot}{R}
\newcommand{\ctrl}{\textup{ctl}}
\newcommand{\received}[1]{\subscr{#1}{rcvd}}
\newcommand{\sensed}[1]{\subscr{#1}{snsd}}
\newcommand{\sampled}[1]{\subscr{#1}{smpld}}
\newcommand{\FCC}[1][]{\mathcal{CC}_{\textup{#1}}}
\newcommand{\ECC}[1][]{\mathcal{ECC}_{\textup{#1}}}
\newcommand{\SFC}[1][]{\mathcal{RSC}_{\textup{#1}}}
\newcommand{\task}[1][]{\mathcal{T}_{\textup{#1}}}

%% Systems Names -- polish following names: why are there 2 for each shit?
\newcommand{\disk}{disk}
\newcommand{\rdisk}{\textup{disk}}
\newcommand{\circledisk}{circle}
\newcommand{\umax}{\subscr{u}{max}}
\newcommand{\rIdisk}{$\infty$-disk}
\newcommand{\LD}{\textup{LD}}
\newcommand{\visdisk}{vis-disk}

\newcommand{\rs}[1]{\supscr{#1}{rs}}

%% FCC Names
\newcommand{\agreepursueName}{\algofont{agree \& pursue}\xspace}
\newcommand{\agreepursue}{\algofont{agree \& pursue}} %% why two?
\newcommand{\agreepursueModName}{\algofont{mod-agree \& pursue}\xspace}

\newcommand{\VicsekName}{\algofont{averaging}\xspace}
\newcommand{\circumcenter}{\algofont{crcmcntr}\xspace}
\newcommand{\nonconvexcircumcenter}{\algofont{nonconvex crcmcntr}\xspace}
\newcommand{\sensorcircumcenter}{\algofont{relative-sensing crcmcntr}\xspace}
\newcommand{\nonconvexsensorcircumcenter}{\algofont{nonconvex relative-sensing crcmcntr}\xspace}

\newcommand{\parallelcircumcenter}{\algofont{pll-crcmcntr}\xspace}
\newcommand{\parallelccenter}[1]{\operatorname{PCC}(#1)}

\newcommand{\VoronoiCentroid}{\algofont{Vrn-cntrd}\xspace}
\newcommand{\VoronoiCentroidDynamics}{\algofont{Vrn-cntrd-dynmcs}\xspace}
\newcommand{\LimitedVoronoiNormal}{\algofont{Lmtd-Vrn-nrml}\xspace}
\newcommand{\LimitedVoronoiCentroid}{\algofont{Lmtd-Vrn-cntrd}\xspace}
\newcommand{\sensorLimitedVoronoiCentroid}{\algofont{relative-sensing Lmtd-Vrn-cntrd}\xspace}
\newcommand{\RangeVoronoiCentroid}{\algofont{Rng-Vrn-cntrd}\xspace}
\newcommand{\VoronoiCircumcenter}{\algofont{Vrn-crcmcntr}\xspace}
\newcommand{\VoronoiIncenter}{\algofont{Vrn-ncntr}\xspace}

%% Task Names
\newcommand{\equidistance}{eqdstnc}

%% Sensor-based networks
\newcommand{\wrt}[2]{ \subscr{#1}{#2} }
\newcommand{\what}[2]{ \supscr{#1}{#2} }

%% Costs
\newcommand{\MCC}{\operatorname{MCC}}
\newcommand{\TCC}{\operatorname{TCC}}
\newcommand{\cc}{\operatorname{IH-MCC}}
\newcommand{\unidir}{\operatorname{unidir}}
\newcommand{\omnidir}{\operatorname{omnidir}}
\newcommand{\nonnllmsgs}{{cmm$\setminus\emptyset$}}
\newcommand{\CommCost}[1][]{\subscr{\operatorname{C}}{rnd}^{#1}}


%%% more about the agree and pursue
\newcommand{\dm}{\mytt{dir}}
\newcommand{\newdm}{\mytt{new-dir}}
\newcommand{\csym}{\mytt{c}}
\newcommand{\ccsym}{\mytt{cc}}
\newcommand{\kprop}{\subscr{k}{prop}}
\newcommand{\Hset}{H}%
\newcommand{\nHset}{n_H}%

%%% random definitions
\newcommand{\fl}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\argmin}{\ensuremath{\operatorname{argmin}}}
\newcommand{\argmax}{\ensuremath{\operatorname{argmax}}}
\newcommand{\arginf}{\ensuremath{\operatorname{arginf}}}
\newcommand{\argsup}{\ensuremath{\operatorname{argsup}}}
\newcommand{\myboolean}{\ensuremath{\{\true,\false\}}} %%to erase

\newcommand{\WW}{{\mathcal{W}}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\Pc}{{\mathcal{P}}}
\newcommand{\reschedule}[3]{{#1}_{(#2,#3)}}
\newcommand{\newC}{\CommCost[]\circ\MM}
\newcommand{\Infnorm}[1]{\|#1\|_{\infty}}

%% symbols for Chp5: rendezvous

%% connectivity maintenance
\newcommand{\XConstrSet}{\mathcal{X}}
\newcommand{\XConstrSetVis}{\subscr{\mathcal{X}}{\visdisk}}
\newcommand{\XConstrSetClessVis}{\subscr{\mathcal{X}}{lc-\visdisk}}

%%\newcommand{\Dc}{\subscr{\UConstrSet}{constraint}}
%%\newcommand{\UConstrSet}{\mathcal{U}}
%%\newcommand{\UConstrSetVis}{\subscr{\mathcal{U}}{\visdisk}}

\newcommand{\rendezvous}{rndzvs}
\newcommand{\ccsalgo}{\algofont{iterated truncation}\xspace}
\newcommand{\rsccsalgo}{\algofont{relative-sensing iterated truncation}\xspace}
\newcommand{\average}{\operatorname{avrg}}
\newcommand{\vers}{\operatorname{vers}}
\newcommand{\piSpace}[1]{\pi_{#1}}


\newcommand{\maximize}{\text{maximize}}
\newcommand{\subj}{\text{subject to}}

\newcommand{\mynum}[1]{{\small\ensuremath{{\texttt{#1}}}\xspace}}

\newcommand{\EE}{\mathcal{E}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\FF}{\mathcal{F}}

%% copyright
\newcommand\reg{$^{\textrm{\tiny\textregistered}}$\xspace}

%% packages for Chp5

\usepackage{psfrag}

%% symbols for Chp 6: Deployment

\newcommand{\deployment}{dply}
\newcommand{\deploymentdistor}{distor-\deployment}
\newcommand{\deploymentarea}{area-\deployment}
\newcommand{\deploymentmixed}{distor-area-\deployment}
\newcommand{\deploymentdc}{dc-\deployment}
\newcommand{\deploymentdcwk}{dc-wk-deployment}
\newcommand{\deploymentsp}{sp-\deployment}
\newcommand{\deploymentspwk}{sp-wk-deployment}

\newcommand{\fcase}[1]{\ensuremath{(\mathbf{#1})}\xspace}
\newcommand{\Pave}{\subscr{P}{ave}}

\newcommand{\centrd}{centrd}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\incenVor}{incntr-Vor}
\newcommand{\circumVor}{crcntr- Vor}

%% symbols for Chp 7: estimation
\newcommand{\Kstf}[1]{\subscr{\supind{K}{#1}}{stf}}
\newcommand{\Kstfna}{\subscr{K}{stf}}

\newcommand{\nip}{\subscr{n}{ip}}
\newcommand{\pdistance}{\mathcal{D}_\lambda}
\newcommand{\arclengthdist}{\subscr{\mathcal{D}}{arc}}
\newcommand{\kapadistance}{\subscr{\mathcal{D}}{curvature}}

\newcommand{\nw}{\mytt{nxt}}
\newcommand{\nwrec}{\mytt{nxtrec}}
\newcommand{\curves}{\mathcal{C}}
\newcommand{\mypath}{\mytt{path}}
\newcommand{\tpath}{\mytt{t}_\mytt{path}}
\newcommand{\tangentat}{\mytt{tangentat}}
\newcommand{\cyclicbalance}{\mytt{cyclic-balance}}
\newcommand{\perpproj}{\mytt{perp-proj}}
\newcommand{\sat}{\operatorname{sat}}
\newcommand{\inclusion}{\operatorname{\iota}}

\newcommand{\eul}{\textsc{Single-Robot Estimate Update Law}\xspace}
\newcommand{\ceul}{\textsc{Cooperative Estimate Update Law}\xspace}
\newcommand{\eupl}{\textsc{Estimate Update and Balancing Law}\xspace}
\newcommand{\aupl}{\textsc{Approximate Estimate and Balancing Law}\xspace}

%% %% OLD ??
%% \newcommand{\optplace}{\mytt{opt-place}}

%% \newcommand{\lw}{\mytt{L}}
%% \newcommand{\setpath}{\operatorname{path}}
%% \newcommand{\regionest}{\mytt{\polygon}}

%% \newcommand{\timewindow}{\mytt{t}}
%% \newcommand{\prev}{\mytt{qprev}}
%% \newcommand{\apdistance}{\mytt{d}}


%% \newcommand{\forget}{\mytt{forget}}

\newcommand{\arclengthparam}{\subscr{s}{arc}}
\newcommand{\gammaarc}{\subscr{\gamma}{arc}}
% \newcommand{\arclength}{\subscr{\gamma}{arc}}
\newcommand{\gammapolar}{\subscr{\gamma}{polar}}
\newcommand{\sign}{\operatorname{sign}}

\newcommand{\Vc}{{\mathscr{V}}}
\newcommand{\Wc}{{\mathscr{W}}}
\newcommand{\Tc}{{\mathscr{T}}}
\newcommand{\Cc}{{\mathscr{C}}}
\newcommand{\Ec}{{\mathscr{E}}}
\newcommand{\DD}{{\mathcal{D}}}
\newcommand{\UU}{{\mathcal{U}}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\ip}{{\mytt{q}}}
\newcommand{\SeqNorm}[1]{\|#1\|_{2,\infty}}
\newcommand{\classK}{\ensuremath{\mathcal{K}}}
\newcommand{\classKinfty}{\ensuremath{\mathcal{K}_{\infty}}}
\newcommand{\classKL}{\ensuremath{\mathcal{KL}}}
\newcommand{\NearNeigh}{\text{NN}}
\newcommand{\NatNeigh}{\text{Nat}}
\newcommand{\triangular}{\text{TIN}}
\newcommand{\inverse}{\text{IDW}}
\newcommand{\localinv}{\text{LIDW}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\MSE}{\operatorname{MSE}}

\newcommand{\Tmin}{\subscr{T}{min}}
\newcommand{\ymin}{\subscr{y}{min}}
\newcommand{\xfree}{\supscr{x}{free}}
\newcommand{\xctrl}{\supscr{x}{ctrl}}

%\renewcommand{\ymaxmin}{\subscr{y}{M-m}}
\newcommand{\Aerr}{\subscr{F}{err}}
\newcommand{\cerr}{\subscr{c}{err}}
\newcommand{\Derr}{\subscr{D}{err}}
\newcommand{\Dave}{\subscr{D}{ave}}
\newcommand{\yerrtilde}{\subscr{\tilde{y}}{err}}

\setlength{\tabcolsep}{3pt}

